Multiple testing when many $p$-values are uniformly conservative, with application to testing qualitative interaction in educational interventions

In the evaluation of treatment effects, it is of major policy interest to know if the treatment is beneficial for some and harmful for others, a phenomenon known as qualitative interaction. We formulate this question as a multiple testing problem with many conservative null $p$-values, in which the classical multiple testing methods may lose power substantially. We propose a simple technique---conditioning---to improve the power. A crucial assumption we need is uniform conservativeness, meaning for any conservative $p$-value $p$, the conditional distribution $(p/\tau)\,|\,p \le \tau$ is stochastically larger than the uniform distribution on $(0,1)$ for any $\tau$. We show this property holds for one-sided tests in a one-dimensional exponential family (e.g.\ testing for qualitative interaction) as well as testing $|\mu|\le\eta$ using a statistic $X \sim \mathrm{N}(\mu,1)$ (e.g.\ testing for practical importance with threshold $\eta$). We propose an adaptive method to select the threshold $\tau$. Our theoretical and simulation results suggest the proposed tests gain significant power when many $p$-values are uniformly conservative and lose little power when no $p$-value is uniformly conservative. We apply our method to two educational intervention datasets.

==> old/theory.tex <==
\section{Theory}
\label{sec:theory}

\newcommand\scan{\text{scan}}
%\wjs{There is some inconsistency in notation. Shall we always use $c$ or $\tau_0$ to denote the cutoff?}

% Let $\hat F_n(\tau)$ be the empirical distribution of $p_1, \ldots, p_n$. That is,
% \[
% \hat F_n(\tau) = \frac{\#\{i: p_i \le \tau\}}{n}.
% \]

\subsection{Theory for conditional tests}
\label{sec:theory-cond-tests}



\subsection{Theory for scan conditional tests}
\label{sec:theory-scan-cond}


\begin{theorem}
The scan conditional test controls type I error for testing the global null under independence.
\end{theorem}
\wjs{This theorem might be correct but highly nontrivial.}


The rest part of this section demonstrates that this scan test is superior compared with the conventional one.

\begin{lemma}\label{lm:simple_mtgl}
Let $U_1, U_2, \ldots, U_n$ be iid uniform random variables on $(0, 1)$ and denote by $\hat F_{U}$ the empirical distribution. Then for any $c > 0$ and $0 < \tau_0 < 1$, we have
\[
\mathbb{P}\left( \max_{\tau > \tau_0} | \hat F_U(\tau)/\tau - 1 | > c \right) \le \frac1{\tau_0 c^2 n}
\]
\end{lemma}


\begin{proof}[Proof of Lemma \ref{lm:simple_mtgl}]
Denote by $\xi_\tau = \frac{\hat F_n(\tau)}{\tau}$. It is well-known that $\xi_\tau$ is a martingale in backward time. Hence, by applying Doob's martingale inequality, we get
\[
\mathbb{P}\left( \max_{\tau > \tau_0} |\hat F_U(\tau)/\tau - 1 | > c \right) \le\frac{\mathbb{E} (\frac{\hat F_U(\tau_0)}{\tau_0} - 1)^2}{c^2} = \frac{1 - \tau_0}{n \tau_0 c^2} < \frac1{\tau_0 c^2 n}.
\]
\end{proof}


Let $\tau_0 > 0$ be a constant. Consider the `$p$'-value adjusted by scanning:
\[
p_{\scan} := \min_{\tau > \tau_0} \frac{p_{\min} |\mathcal S_{\tau}|}{\tau n}.
\]
The global null is rejected if 
\[
n \cdot p_{\scan} < \alpha_{\scan}
\]
for some constant $\alpha_{\scan}$, which is given by simulations.
% Let $p_1, p_2, \ldots, p_n$ be (one-sided or two-sided) $p$-values for testing the normal means problem $y \sim \mathcal{N}(\bm\mu, \sigma^2 \bm I_n)$ with variance $\sigma^2$ known. Write $\mu_i = c_i \sigma \sqrt{2\log p}$
\begin{theorem}\label{thm:same_power}
% Let $\tau_0 > 0$ be a constant. Let $p_1, p_2, \ldots, p_n$ be (one-sided or two-sided) $p$-values for testing the normal means problem $y \sim \mathcal{N}(\bm\mu, \sigma^2 \bm I_n)$ with variance $\sigma^2$ known. If the mean vector $\bm\mu$ has exactly one nonzero component under alternative, then the conditional Bonferroni test has the same power as the conventional Bonferroni test: that is, they both have power one if the nonzero component exceeds $\sigma (1 + \epsilon)\sqrt{2\log n}$; or both are powerless if it is below $\sigma (1 - \epsilon)\sqrt{2\log n}$, where $\epsilon > 0$ is any arbitrary constant. In other words, they have (asymptotically) the same threshold for a given target type I error.
Suppose all the $p$-values are jointly independent and $\tau_0, \alpha < 1$ are two positive constants. As $n \rightarrow \infty$, the scan conditional Bonferroni test at level $\alpha$ is asymptotically more powerful than the conventional one at level $\alpha + o(1)$.
\end{theorem}
\begin{proof}[Proof of Theorem \ref{thm:same_power}]
First note that
\[
n \cdot p_{\scan} = n \min_{\tau > \tau_0} \frac{p_{\min} |\mathcal S_{\tau}|}{\tau n} \le \frac{p_{\min} |\mathcal S_{1}|}{1} = n p_{\min},
\]
which is the test statistic used in the conventional Bonferroni test. If we can show that $\alpha_{\scan} \ge \alpha - o(1)$, the proof is complete. To see this, 

Apply Lemma \ref{lm:simple_mtgl}.
\end{proof}

We will soon be interested in scenarios where the conditional test is strictly more powerful than the conventional one. Suppose only a vanishing fraction of the $p$-values are false null. Among the true nulls, a constant fraction are strictly stochastically larger than uniform on $(0,1)$ and the rest are uniform on $(0,1)$. Then the following theorem concludes that conditioning indeed pays off.

\begin{theorem}\label{thm:more_power}
Under the preceding conditions, the conditional test is more powerful.
\end{theorem}

\begin{proof}[Proof of Theorem \ref{thm:more_power}]
Use the fact that
\[
\inf_{\tau > \tau_0 } \frac{\hat F_n(\tau)}{\tau}
\]
is strictly smaller than 1.

\end{proof}



Can we develop some theoretical results?

We can start with Bonferroni and the needle-in-a-haystack setting. I
did some heuristic calculation for the scan conditional Bonferroni for
some fixed $\epsilon > 0$
\[
p^{*} = \inf_{\tau > \tau_0}\, n p_{(1)} \cdot \hat{F}_n(\tau)/\tau.
\]
We can show $\hat{F}_n(\tau)/\tau \to 1$ uniformly if the $p$-values
are all uniform, so the rejection region is almost $p^{*} < \alpha$.

I think we can show the detection threshold in the needle in
the needle-in-a-haystack setting is
\[
\sqrt{2 \log (n \cdot \inf_{\tau > \tau_0} F(\tau)/\tau)},
\]
where $F$ is the distribution of null $p$-values (possibly
conservative). When $F$ is very conservative, $\inf_{\tau > \tau_0}
F(\tau)/\tau$ is much smaller than $1$.

The question is: in what sense is this detection threshold optimal?
Another related question is: so far we need $\tau_0$ fixed, but in
some cases (e.g.\ normal mean problem) $F(\tau)/\tau \to 0$ as $\tau
\to 0$. So it seems we can do better by not requiring $\tau >
\tau_0$.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

